SpamDam: Towards Privacy-Preserving and Adversary-Resistant SMS Spam Detection

In this study, we introduce SpamDam, a SMS spam detection framework designed to overcome key challenges in detecting and understanding SMS spam, such as the lack of public SMS spam datasets, increasing privacy concerns of collecting SMS data, and the need for adversary-resistant detection models. SpamDam comprises four innovative modules: an SMS spam radar that identifies spam messages from online social networks(OSNs); an SMS spam inspector for statistical analysis; SMS spam detectors(SSDs) that enable both central training and federated learning; and an SSD analyzer that evaluates model resistance against adversaries in realistic scenarios. Leveraging SpamDam, we have compiled over 76K SMS spam messages from Twitter and Weibo between 2018 and 2023, forming the largest dataset of its kind. This dataset has enabled new insights into recent spam campaigns and the training of high-performing binary and multi-label classifiers for spam detection. Furthermore, effectiveness of federated learning has been well demonstrated to enable privacy-preserving SMS spam detection. Additionally, we have rigorously tested the adversarial robustness of SMS spam detection models, introducing the novel reverse backdoor attack, which has shown effectiveness and stealthiness in practical tests.

==> 0_abstract.tex <==
In this study, we introduce \textit{SpamDam}, a SMS spam detection framework designed to overcome key challenges in detecting and understanding SMS spam, such as the lack of public SMS spam datasets, increasing privacy concerns of collecting SMS data, and the need for adversary-resistant detection models. \textit{SpamDam} comprises four innovative modules: an SMS spam radar that identifies spam messages from online social networks(OSNs); an SMS spam inspector for statistical analysis; SMS spam detectors(SSDs) that enable both central training and federated learning; and an SSD analyzer that evaluates model resistance against adversaries in realistic scenarios.

Leveraging \textit{SpamDam}, we have compiled over 76K SMS spam messages from Twitter and Weibo between 2018 and 2023, forming the largest dataset of its kind. This dataset has enabled new insights into recent spam campaigns and the training of high-performing binary and multi-label classifiers for spam detection. Furthermore, effectiveness of federated learning has been well demonstrated to enable privacy-preserving SMS spam detection. Additionally, we have rigorously tested the adversarial robustness of SMS spam detection models, introducing the novel \textit{reverse backdoor attack}, which has shown effectiveness and stealthiness in practical tests.

==> 0_main.tex <==


\section{Introduction}
\label{sec:intro}
\input{1_intro}

\section{Background and Related Works}
\label{sec:background}
\input{2_background}
%
\section{The Discovery and Characterization of SMS Spam}
\label{sec:method}
\input{3_data_collection.tex}
%
\section{The Classification of SMS Spam}
\label{sec:spam_detection}
\input{4_spam_detection.tex}
%
\section{The Adversarial Resistance of SMS Spam Classification}
\label{sec:adversary}
\input{5_1_adversarial_robustness.tex}



\section{Discussion}
\label{sec:discuss}
\input{6_discussion.tex}
%


\section{Conclusion}
\label{sec:conclusion}
\input{8_conclusion}

==> author.tex <==
\author[1]{Yekai Li}
\author[1]{Rufan Zhang}
\author[1]{Wenxin Rong}
\author[1]{Xianghang Mi}

\affil[1]{University of Science and Technology of China}

\affil[ ]{\url{https://chasesecurity.github.io/SpamDam}}

\renewcommand*{\Affilfont}{\small\it}
\IEEEoverridecommandlockouts



==> commons/commands.tex <==

\newcommand{\revised}[2]{
    \textcolor{red}{\sout{#1}}\textcolor{blue}{#2}
}
\newcommand{\arevised}[1]{\textcolor{blue}{#1}}
\newcommand{\mrevised}[1]{\textcolor{magenta}{#1}}
\newcommand{\qrevised}[1]{\textcolor{cyan}{#1}}
\newcommand{\drevised}[1]{\sout{#1}}
% once draft is ready, 
% \renewcommand{\revised}[1]{#1}
% \renewcommand{\arevised}[1]{#1}
% \renewcommand{\mrevised}[1]{#1}
% \renewcommand{\qrevised}[1]{#1}
% \renewcommand{\drevised}[1]{}
\newcommand{\xmi}[1]{\textcolor{red}{\textbf{xmi:} #1}}
\newcommand{\yekai}[1]{\textcolor{brown}{\textbf{yekai:} #1}}
\newcommand{\rufan}[1]{\textcolor{blue}{\textbf{rufan:} #1}}
\newcommand{\subject}[1]{\vspace{3pt}\noindent\textbf{#1}}
\newcommand{\subsubject}[1]{\vspace{3pt}\noindent\textit{#1}}

%\renewcommand{\thefootnote}{\fnsymbol{footnote}}
%\footnotetext[1]{Corresponding author.}

%
%\newcommand\malurl[1]{\href{notalink}{\textcolor{blue}{\nolinkurl{#1}}}}
\newcommand\malurl[1]{\href{notalink}{{\nolinkurl{#1}}}}
% the finding box
\newcounter{finding}
\setcounter{finding}{1}
\newcommand{\finding}[1]{
\vspace{3pt}
\noindent
\framebox{
\begin{minipage}[b]{3.3in}
\noindent \textbf{Finding \Roman{finding}}: \textit{#1}
\stepcounter{finding}
\end{minipage}
}
\vspace{-5pt}
}

\newcommand{\ignore}[1]{}

\newcommand{\radar}{\textit{SpamRadar}}

\newcommand{\hunter}{\textit{SpamHunter}}
\newcommand{\mathv}[2]{\ensuremath{\text{#1}_\mathsf{#2}}}

% When generating the axiv version with more content, let's set this value as 1
\def\arxiv{1}

==> commons/pkgs.tex <==
\usepackage[utf8]{inputenc}
% it, be sure to load this package with the cmex10 option to ensure that
% only type 1 fonts will utilized at all point sizes. Without this option,
% it is possible that some math symbols, particularly those within
% footnotes, will be rendered in bitmap form which will result in a
% document that can not be IEEE Xplore compliant!
\usepackage{amsmath}
\usepackage{graphicx}
% it is a good idea to load it with the tight package option to reduce
% the amount of white space around the subfigures. 
\usepackage[tight,footnotesize]{subfigure}
%\usepackage[caption=false,font=footnotesize]{subfig}
\usepackage{multirow}
\usepackage{fancyvrb}
\usepackage[flushleft, online]{threeparttable}
% Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space,
\usepackage{cite}
\usepackage{xurl}
\usepackage[
    colorlinks,
    linkcolor=blue,
    anchorcolor=blue,
    citecolor=blue,
    urlcolor=blue
]{hyperref}
\usepackage{array}
\usepackage{algorithmic}
\usepackage{booktabs}
\usepackage{xcolor}
\usepackage{cite}
\usepackage{authblk}

==> title.tex <==
\title{Towards Privacy-Preserving and Adversary-Resistant SMS Spam Detection}
\title{SpamDam: Towards Privacy-Preserving and Adversary-Resistant SMS Spam Detection}
